Adaptive Contrastive Search: Uncertainty-Guided Decoding for Open-Ended Text Generation

Decoding from the output distributions of large language models to produce high-quality text is a complex challenge in language modeling. Various approaches, such as beam search, sampling with temperature, $k-$sampling, nucleus $p-$sampling, typical decoding, contrastive decoding, and contrastive search, have been proposed to address this problem, aiming to improve coherence, diversity, as well as resemblance to human-generated text. In this study, we introduce adaptive contrastive search, a novel decoding strategy extending contrastive search by incorporating an adaptive degeneration penalty, guided by the estimated uncertainty of the model at each generation step. This strategy is designed to enhance both the creativity and diversity of the language modeling process while at the same time producing coherent and high-quality generated text output. Our findings indicate performance enhancement in both aspects, across different model architectures and datasets, underscoring the effectiveness of our method in text generation tasks. Our code base, datasets, and models are publicly available.

==> fig_tables/case_study_2.tex <==
\begin{tabular}{|c|c|c|c|}
\hline prompt & \begin{tabular}{l} 
Butt criticized Donald's controls in certain situations in the game, as well as the difficulty \\
of some levels and puzzles. Buchanan also criticized the controls, calling
\end{tabular} & div. & coh. \\
\hline beam & \begin{tabular}{l} 
them " too easy " and " too difficult ". He also criticized the game's graphics, stating that the game's \\
graphics were " too simplistic " and "too simplistic ". He also criticized the game's graphics, stating \\
that the game's graphics were " too simplistic" and " too simplistic ". He also criticized the graphics, \\
stating that the game's graphics were " too simplistic " and " too simplistic ". He also criticized the \\
graphics, stating that the game's graphics were " too simplistic " and " too simplistic ". He also \\
criticized the graphics, stating that the game's graphics were"...
\end{tabular} & 0.02 & 0.605  \\
\hline nucleus & \begin{tabular}{l} 
them " offensively rudimentary ". After the game was released, Buchanan wrote a number of game \\
reviews about his review of the game, primarily summarizing what he thought the reviewers had \\
enjoyed about it. Buchanan was pleased with how consistently these reviews awarded the game. \\
For one, he praised the puzzles, compared them to Nos. 1 and 2 and enjoyed the construction of the \\
artificial intelligence in the game's forms. He found no fault with the puzzles, even in those situations \\
where they seemed repetitive. According to an Xbox Magazine review, " every time...
\end{tabular} & 0.98 & 0.597  \\
\hline contrastive decoding & \begin{tabular}{l} 
them " unimpressive " and a " nightmare " of an experience to play with players unfamiliar with \\
Tetris. On the other hand, his opinion was shared by other reviewers, and some were critical of the \\
game's technical design for the Wii version of Tetris. In addition, Tintin's review included a quote \\
from Roger Ebert, who said that Tetris was better than the original game due to its simplicity and \\
ease of play. Ebert's comments were included in the game's DVD commentary, released on March \\
22,2010 . It is unclear if any of the video commentary was taken from ...
\end{tabular} & 0.98 & 0.626  \\
\hline contrastive search & \begin{tabular}{l} 
them " unimpressive " and a " nightmare " of an experience to play with players unfamiliar with \\
Tetris. On the other hand, his opinion was shared by other reviewers, and some were critical of the \\
game's technical design for the Wii version of Tetris. In addition, Tintin's review included a quote \\
from Roger Ebert, who said that Tetris was better than the original game due to its simplicity and \\
ease of play. Ebert's comments were included in the game's DVD commentary, released on March \\
22,2010 . It is unclear if any of the video commentary was taken from ...
\end{tabular} & 0.98 & 0.626  \\
\hline adaptive cs & \begin{tabular}{l} 
them " unimpressive " and a " nightmare " of an experience to play with players unfamiliar with \\
Tetris. On the other hand, his opinion was shared by other reviewers, and some were critical of the \\
game's technical design for the Wii version of Tetris. In addition, Tintin's review included a quote \\
from Roger Ebert, who said that Tetris was better than the original game due to its simplicity and \\
ease of play. Ebert's comments were included in the game's DVD commentary, released on March \\
22,2010 . It is unclear if any of the video commentary was taken from ...
\end{tabular} & 0.98 & 0.626  \\



\hline
\end{tabular}



==> fig_tables/case_study_3.tex <==
\begin{tabular}{|c|c|c|c|c|}
\hline prefix & \begin{tabular}{l} 
Butt criticized Donald's controls in certain situations in the game, as well as the difficulty \\
of some levels and puzzles. Buchanan also criticized the controls, calling
\end{tabular} & div. & coh. & gen-ppl \\
\hline beam & \begin{tabular}{l} 
them " too easy " and " too difficult ". He also criticized the game's graphics, stating that the game's \\
graphics were " too simplistic " and "too simplistic ". He also criticized the game's graphics, stating \\
that the game's graphics were " too simplistic" and " too simplistic ". He also criticized the graphics, \\
stating that the game's graphics were " too simplistic " and " too simplistic ". He also criticized the \\
graphics, stating that the game's graphics were " too simplistic " and " too simplistic ". He also \\
criticized the graphics, stating that the game's graphics were"...
\end{tabular} & 0.02 & 0.605 & 7.91 \\
\hline nucleus & \begin{tabular}{l} 
them " offensively rudimentary ". After the game was released, Buchanan wrote a number of game \\
reviews about his review of the game, primarily summarizing what he thought the reviewers had \\
enjoyed about it. Buchanan was pleased with how consistently these reviews awarded the game. \\
For one, he praised the puzzles, compared them to Nos. 1 and 2 and enjoyed the construction of the \\
artificial intelligence in the game's forms. He found no fault with the puzzles, even in those situations \\
where they seemed repetitive. According to an Xbox Magazine review, " every time...
\end{tabular} & 0.98 & 0.597 & 37.83 \\
\hline contrastive decoding & \begin{tabular}{l} 
them " unimpressive " and a " nightmare " of an experience to play with players unfamiliar with \\
Tetris. On the other hand, his opinion was shared by other reviewers, and some were critical of the \\
game's technical design for the Wii version of Tetris. In addition, Tintin's review included a quote \\
from Roger Ebert, who said that Tetris was better than the original game due to its simplicity and \\
ease of play. Ebert's comments were included in the game's DVD commentary, released on March \\
22,2010 . It is unclear if any of the video commentary was taken from ...
\end{tabular} & 0.98 & 0.626 & 19.64 \\
\hline contrastive search & \begin{tabular}{l} 
them " unimpressive " and a " nightmare " of an experience to play with players unfamiliar with \\
Tetris. On the other hand, his opinion was shared by other reviewers, and some were critical of the \\
game's technical design for the Wii version of Tetris. In addition, Tintin's review included a quote \\
from Roger Ebert, who said that Tetris was better than the original game due to its simplicity and \\
ease of play. Ebert's comments were included in the game's DVD commentary, released on March \\
22,2010 . It is unclear if any of the video commentary was taken from ...
\end{tabular} & 0.98 & 0.626 & 19.64 \\
\hline adaptive cs & \begin{tabular}{l} 
them " unimpressive " and a " nightmare " of an experience to play with players unfamiliar with \\
Tetris. On the other hand, his opinion was shared by other reviewers, and some were critical of the \\
game's technical design for the Wii version of Tetris. In addition, Tintin's review included a quote \\
from Roger Ebert, who said that Tetris was better than the original game due to its simplicity and \\
ease of play. Ebert's comments were included in the game's DVD commentary, released on March \\
22,2010 . It is unclear if any of the video commentary was taken from ...
\end{tabular} & 0.98 & 0.626 & 19.64 \\



\hline
\end{tabular}



==> fig_tables/results_merged_test.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline \multirow{2}{*}{ Model } & \multicolumn{4}{|c|}{ Language Modelling Quality } & \multirow[b]{2}{*}{ Method } & \multicolumn{7}{|c|}{ Generation Quality } \\
 & $\mathrm{ppl} \downarrow$ & $\operatorname{acc} \uparrow$ & rep $\downarrow$ & wrep $\downarrow$ & & rep- $2 \downarrow$ & rep- $3 \downarrow$ & rep- $4 \downarrow$ & diversity $\uparrow$ & MAUVE $\uparrow$ & coherence $\uparrow$ & gen-ppl \\
\hline \multirow{5}{*}{ MLE } & \multirow{5}{*}{24.32} & \multirow{5}{*}{39.63} & \multirow{5}{*}{52.82} & \multirow{5}{*}{29.97} & greedy & 69.21 & 65.18 & 62.05 & 0.04 & 0.03 & 0.587 & 7.32 \\
 & & & & & beam & 71.94 & 68.97 & 66.62 & 0.03 & 0.03 & 0.585 & 6.42 \\
 & & & & & nucleus & 4.45 & 0.81 & 0.43 & 0.94 & 0.90 & 0.577 & 49.71 \\
 & & & & & contrastive & 44.20 & 37.07 & 32.44 & 0.24 & 0.18 & 0.599 & 9.90 \\
& & & & & adaptive cs & 44.20 & 37.07 & 32.44 & 0.24 & 0.18 & 0.599 & 9.90 \\
\hline \multirow{5}{*}{ Unlike. } & \multirow{5}{*}{28.57} & \multirow{5}{*}{38.41} & \multirow{5}{*}{51.23} & \multirow{5}{*}{28.57} & greedy & 24.12 & 13.35 & 8.04 & 0.61 & 0.69 & 0.568 & 37.82 \\
 & & & & & beam & 11.83 & 5.11 & 2.86 & 0.81 & 0.75 & 0.524 & 34.73 \\
 & & & & & nucleus & 4.01 & 0.80 & 0.42 & 0.95 & 0.87 & 0.563 & 72.03 \\
 & & & & & contrastive & 7.48 & 3.23 & 1.40 & 0.88 & 0.83 & 0.574 & 43.61 \\
  & & & & & adaptive cs & 7.48 & 3.23 & 1.40 & 0.88 & 0.83 & 0.574 & 43.61 \\
\hline \multirow{5}{*}{ SimCTG } & \multirow{5}{*}{23.82} & \multirow{5}{*}{40.91} & \multirow{5}{*}{51.66} & \multirow{5}{*}{28.65} & greedy & 67.36 & 63.33 & 60.17 & 0.05 & 0.05 & 0.596 & 7.16 \\
 & & & & & beam & 70.32 & 67.17 & 64.64 & 0.04 & 0.06 & 0.591 & 6.36 \\
 & & & & & nucleus & 4.05 & 0.79 & 0.37 & 0.94 & 0.92 & 0.584 & 47.19 \\
 & & & & & contrastive & 3.93 & 0.78 & 0.31 & 0.95 & 0.94 & 0.610 & 18.26 \\
  & & & & & adaptive cs & 3.93 & 0.78 & 0.31 & 0.95 & 0.94 & 0.610 & 18.26 \\
\hline Human & - & - & 36.19 & - & - & 3.92 & 0.88 & 0.28 & 0.95 & 1.00 & 0.644 & 24.01 \\
\hline
\end{tabular}
